Nonparametric gamma kernel estimators of density derivatives on positive semiaxis

We consider nonparametric estimation of the derivative of a probability density function with the bounded support on $[0,\infty)$. Estimates are looked up in the class of estimates with asymmetric gamma kernel functions. The use of gamma kernels is due to the fact they are nonnegative, change their shape depending on the position on the semi-axis and possess other good properties. We found analytical expressions for bias, variance, mean integrated squared error (MISE) of the derivative estimate. An optimal bandwidth, the optimal MISE, and rate of mean square convergence of the estimates for density derivative have also been found.

==> reference.tex <==
@InProceedings{Bonald,
author = {T. Bonald and L. Massouli\'{e} and F. Mathieu and D. Perino and A. Twigg},
title = {Epidemic Live Streaming: Optimal Performance Trade-Offs},
booktitle = {Proc. of ACM SIGMETRICS 2008},
OPTcrossref = {},
OPTkey = {},
pages = {325-336},
year = {2008},
OPTeditor = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTmonth = {},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@Article{ColesTawn,
author = {Coles S., Heffernan J., Tawn J.},
title = {Dependence Measures for Extreme Value Analysis},
journal = {Extremes},
year = {1999},
OPTkey = {},
volume = {2},
number = {4},
pages = {339-365},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@Article{Dan,
author = {G. D\'{a}n and V. Fodor},
title = {Delay Asymptotics and Scalability for Peer-to-peer Live Streaming},
journal = {IEEE Trans. Parallel Distrib.},
year = {2009},
OPTkey = {},
volume = {20},
number = {10},
pages = {1499-1511},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@Article{Auria2,
author = {B.~D'Auria and   S.~I.~Resnick},
title = {The influence of dependence on
data network models of burstiness},
journal = {Adv. Appl. Probab.},
year = {2008},
OPTkey = {},
volume = {40},
OPTnumber = {1},
pages = {60-94},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@Article{DavisResnick,
author = {Davis R.A., Resnick S.I.},
title = {Limit theory for bilinear  processes with heavy tailed noise},
journal = {Ann. Appl. Probab.},
year = {1996},
OPTkey = {},
volume = {*},
OPTnumber = {6},
pages = {1191-1210},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@Book{Embrechts,
author = {P. Embrechts and C. Kl\H{u}ppelberg and T. Mikosch},
ALTeditor = {},
title = {Modeling Extremal Events for Finance and Insurance},
publisher = {Springer, Berlin},
year = {1997},
OPTkey = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@Book{Feller,
author = {W. Feller},
ALTeditor = {},
title = {An Introduction to Probability Theory and Its Applications},
publisher = {Wiley, New York},
year = {1971},
OPTkey = {},
OPTvolume = {2},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {3},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@ARTICLE{Hernandes-Campos,
  AUTHOR =       {Hern\'{a}ndes-Campos F., Marron J.S., Samorodnitsky G. and Smith F.D.},
  TITLE =        {Variable Heavy Tails in Internet Traffic},
  JOURNAL =      {Performance Evaluation},
  YEAR =         {2004},
  volume =       {58},
  number =       {},
  pages =        {261-284},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
}

@ARTICLE{JessenMikosch,
  AUTHOR =       {Jessen A.H., Mikosch T.},
  TITLE =        {Regularly varying functions},
  JOURNAL =      {Publications de L'Institut Math\'{e}matique. Nouvelle s\'{e}rie},
  YEAR =         {2006},
  volume =       {80},
  number =       {94},
  pages =        {171-192},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
}

@Book{Feller,
author = {W. Feller},
ALTeditor = {},
title = {An Introduction to Probability Theory and Its Applications},
publisher = {Wiley, New York},
year = {1971},
OPTkey = {},
OPTvolume = {2},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {3},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@Book{Kalashnikov,
  author =      {Kalashnikov V.},
  ALTeditor = {},
title =        {Geometric Sums: Bounds for Rare Events with Applications},
  publisher =    {Kluwer Academic Publishers},
  year =         {1997},
  OPTkey = {},
OPTvolume = {2},
OPTnumber = {},
OPTseries = {},
OPTaddress =      {Dordrecht-Boston-London},
  OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


%\bibitem{Kalashnikov}
%Kalashnikov V.: Geometric Sums: Bounds for Rare Events with Applications. Dordrecht-Boston-London, Kluwer Academic Publishers, 1997

@TECHREPORT{Klivansky,
  AUTHOR =       {Klivansky S.M., Mukherjee A. and Song C.},
  TITLE =        {On Long-Range Dependence in NSFNET Traffic},
  INSTITUTION =  {Technical Report CIT-CC-94-61},
  YEAR =         {1994},
  type =         {},
  number =       {},
  address =      {},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
}

%\bibitem{Klivansky}
%Klivansky S.M., Mukherjee A., Song C.: On Long-Range Dependence in NSFNET Traffic, Technical Report CIT-CC-94-61, 1994


@BOOK{Markovich-2007,
  AUTHOR =       {Markovich N.M.},
  editor =       {},
  TITLE =        {Nonparametric Estimation of Univariate Heavy-Tailed Data},
  PUBLISHER =    {J. Wiley \& Sons},
  YEAR =         {2007},
  volume =       {},
  number =       {},
  series =       {},
  address =      {Chichester},
  edition =      {},
  month =        {},
  note =         {},
  abstract =     {},
  isbn =         {},
  price =        {},
  keywords =     {},
  source =       {},
}




@Article{MarkKilpi-2009,
author = {Markovich N.M., Kilpi,J.},
title = {Bivariate statistical analysis of TCP-flow sizes and durations},
journal = {Annals of Operations Research},
year = {2009},
OPTkey = {},
volume = {170},
OPTnumber = {1},
pages = {199-216},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@InProceedings{MarkKrieg-2006,
  author =  {Markovich N.M., U.R.Krieger},
  title =        {Statistical Analysis  of VoIP Flows Generated by Skype Users},
  booktitle =    {IEEE International workshop on traffic management and traffic engineering for the future Internet, FITraMEn},
  OPTcrossref = {},
OPTkey = {},
pages = {1-6},
year = {2008},
OPTeditor = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {Porto, Portugal},
OPTmonth = {},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}
 
@Book{Embrechts,
author = {P. Embrechts and C. Kl\H{u}ppelberg and T. Mikosch},
ALTeditor = {},
title = {Modeling Extremal Events for Finance and Insurance},
publisher = {Springer, Berlin},
year = {1997},
OPTkey = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
} 
  
@Inbook{MarkKrieg-2009,
  author =       {Markovich N. M.,   Krieger U. R.},
  ALTeditor = {D.D. Kouvatsos},
title = {Statistical Inspection and Analysis Techniques for Traffic Data Arising from the Internet},
publisher = {River Publishers},
OPTchapter =      {2, Traffic and Performance Engineering for Heterogeneous Networks},
  OPTpages =        {41-60},
year = {2009},
OPTkey = {},
OPTvolume = {1},
OPTnumber = {},
OPTseries = {Series in Information Science and
Technology},
OPTaddress = {},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
} 



%\bibitem{MarkKrieg-2009}
%Markovich N. M.,   Krieger U. R.: Statistical Inspection and Analysis Techniques for Traffic Data Arising from the Internet, Chapter 2, Traffic and %Performance Engineering for Heterogeneous Networks, D.D. Kouvatsos (Ed.), ISBN 978-87-92329-16-5, River Publishers Series in Information Science and
%Technology - Vol. 1, pp. 41-60, 2009


@Article{MarkUnd,
author = {Markovich N. M.,   Undheim A. and   Emstad P.~J.},
title = {Classification of Slice-Based VBR Video  Traffic},
journal = {Comput. Netw.},
year = {2009},
OPTkey = {},
volume = {},
OPTnumber = {53},
pages = {1137-1153},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@Article{MarkKrieg-2010b,
author = {Markovich N.M., Krieger U.R.},
title = {Statistical Analysis and Modeling of Skype VoIP Flows},
journal = {Computer Communications (COMCOM)},
year = {2010},
OPTkey = {},
volume = {31},
OPTnumber = {1},
pages = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

@INBOOK{MarkKrieg-2011,
  AUTHOR =       {Markovich N. M.,   Krieger U. R.},
  editor =       {},
  TITLE =        {Statistical Analysis and Modeling of Peer-to-Peer Multimedia Traffic},
  CHAPTER =      {Performance Handbook SPIN 12440030, LNCS 5233},
  pages =        {},
  PUBLISHER =    {Springer},
  YEAR =         {2010},
  volume =       {},
  number =       {},
  series =       {Lecture Notes in Computer Science,  Next Generation Internet: Performance Evaluation \& Applications},
  type =         {},
  address =      {},
  edition =      {},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
}

 %\bibitem{MarkKrieg-2011}
 %Markovich N. M.,   Krieger U. R.: Statistical Analysis and Modeling of Peer-to-Peer Multimedia Traffic,  In: Performance Handbook SPIN 12440030, LNCS %5233, ISBN 978-3-642-02741-3, Series: Lecture Notes in Computer Science,  Next Generation Internet: Performance Evaluation \& Applications, Springer, %2010

@InProceedings{Markovich-2010,
  author =  {Markovich N.M.},
  title =        {Modeling of Dependence in a Peer-to-Peer Video Application},
  booktitle =    {The 6th International Wireless Communications \& Mobile Computing Conference (IWCMC 2010 TRAC)},
  OPTcrossref = {},
OPTkey = {},
pages = {1-6},
year = {2010},
OPTeditor = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {Caen, France},
OPTmonth = {28.06-2.07.2010},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}

 
@Article{Markovich-2012,
author = {Markovich N.M.},
title = {Quality Assessment of the  Packet Transport  of Peer-to-Peer
        Video Traffic in High-Speed Networks},
journal = {Performance Evaluation},
year = {2012},
OPTkey = {},
volume = {31},
OPTnumber = {1},
pages = {},
OPTmonth = {},
OPTnote = {Accepted, ``unpublished''},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@InProceedings{Massoulie,
author = {L. Massoulie and A. Twigg and C. Gkantsidis and  P. Rodrigues},
title = {Randomized decentralized broadcasting algorithms},
booktitle = {Proc. of IEEE INFOCOM},
OPTcrossref = {},
OPTkey = {},
pages = {1073 - 1081},
year = {2007},
OPTeditor = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTmonth = {},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
doi = {10.1109/INFCOM.2007.129},
issn = {0743-166X},
OPTlocalfile = {},
OPTabstract = {}
}

@Book{Moder,
author = {Moder J.~J.,  Elmaghraby S.~E.},
ALTeditor = {},
title = {Handbook of Operations Research, Foundations and Fundamentals},
publisher = {Van Nostrand Reinhold Company},
year = {1978},
OPTkey = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {New York},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@Book{Resnick,
author = {Resnick S.I.},
ALTeditor = {},
title = {Heavy-Tail Phenomena. Probabilistic and Statistical
Modeling},
publisher = {Springer, New York},
year = {2006},
OPTkey = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
OPTlocalfile = {},
OPTabstract = {}
}


@INBOOK{Testa,
  AUTHOR =       {Testa C., Rossi D., Rao A. and Legout A.},
  editor =       {},
  TITLE =        {Experimental Assessment of BitTorrent Completion Time in Heterogeneous TCP/uTP Swarms.},
  CHAPTER =      {Traffic Monitoring and Analysis,  ISBN 978-3-642-28533-2},
  pages =        {52-65},
  PUBLISHER =    {Springer},
  YEAR =         {2012},
  volume =       {},
  number =       {},
  series =       {Lecture Notes in Computer Science 7189},
  type =         {},
  address =      {},
  edition =      {},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
}

%\bibitem{Testa}
%Testa C., Rossi D., Rao A., Legout A.: Experimental Assessment of BitTorrent Completion Time in Heterogeneous TCP/uTP Swarms. In: Traffic Monitoring %and Analysis,  ISBN 978-3-642-28533-2, Series: Lecture Notes in Computer Science 7189, 52-65, Springer, 2012

@InProceedings{Zaborovsky,
author = {V. Zaborovsky and R. Meylanov},
title = {Peer-to peer fractal models: new
approach to describe multiscale network processes},
booktitle = {Proc. of ICT 2002},
OPTcrossref = {},
OPTkey = {},
pages = {1095-1100},
year = {2002},
OPTeditor = {},
OPTvolume = {1},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTmonth = {},
OPTorganization = {},
OPTpublisher = {},
OPTnote = {},
OPTannote = {},
OPTurl = {},
OPTdoi = {},
OPTissn = {},
localfile = {Beijing, China},
OPTabstract = {}
}

@INBOOK{Wang,
  AUTHOR =       {Wang K., Jiang Y., Lin C.},
  editor =       {},
  TITLE =        {Experimental Assessment of BitTorrent Completion Time in Heterogeneous TCP/uTP Swarms.},
  CHAPTER =      {Measurement, Modelling, and Evaluation of Computing Systems and Dependability and Fault Tolerance,  ISBN 978-3-642-28539-4},
  pages =        {302-316},
  PUBLISHER =    {Springer},
  YEAR =         {2012},
  volume =       {},
  number =       {},
  series =       {Lecture Notes in Computer Science 7201},
  type =         {},
  address =      {},
  edition =      {},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
}
%\bibitem{Wang}
%Wang K., Jiang Y., Lin C.: Modeling and Analysis of a P2P-VoD System Based on Stochastic Network Calculus. In: Measurement, Modelling, and Evaluation %of Computing Systems and Dependability and Fault Tolerance,  ISBN 978-3-642-28539-4, Series: Lecture Notes in Computer Science 7201, 302-316, %Springer, 2012

